Adaptive Question Answering: Enhancing Language Model Proficiency for Addressing Knowledge Conflicts with Source Citations

Resolving knowledge conflicts is a crucial challenge in Question Answering (QA) tasks, as the internet contains numerous conflicting facts and opinions. While some research has made progress in tackling ambiguous settings where multiple valid answers exist, these approaches often neglect to provide source citations, leaving users to evaluate the factuality of each answer. On the other hand, existing work on citation generation has focused on unambiguous settings with single answers, failing to address the complexity of real-world scenarios. Despite the importance of both aspects, no prior research has combined them, leaving a significant gap in the development of QA systems. In this work, we bridge this gap by proposing the novel task of QA with source citation in ambiguous settings, where multiple valid answers exist. To facilitate research in this area, we create a comprehensive framework consisting of: (1) five novel datasets, obtained by augmenting three existing reading comprehension datasets with citation meta-data across various ambiguous settings, such as distractors and paraphrasing; (2) the first ambiguous multi-hop QA dataset featuring real-world, naturally occurring contexts; (3) two new metrics to evaluate models' performances; and (4) several strong baselines using rule-based, prompting, and finetuning approaches over five large language models. We hope that this new task, datasets, metrics, and baselines will inspire the community to push the boundaries of QA research and develop more trustworthy and interpretable systems.

==> generation_example_old.tex <==
\begin{table*}[t]
\centering
\tiny
\setlength{\tabcolsep}{0.3pt}


\renewcommand{\arraystretch}{1}
\begin{tabular}{ccccc}
\textbf{Dataset}          & \textbf{Question}                                                                                                                                 & \textbf{Context}                                                                     & \textbf{\begin{tabular}[c]{@{}c@{}}Zero-shot\\ Answer\end{tabular}}                                                                                                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Few-shot\\ Answer\end{tabular}}                                                                                                                                                                                                                                                 \\ \hline
\multirow{3}{*}{AmbigQA-Cite}  & \begin{tabular}[c]{@{}c@{}}Who played warden\\ hodges in dad's army?\end{tabular}                                                                 & \begin{tabular}[c]{@{}c@{}}{}[...] \textbf{Bill Pertwee} as Hodges [...] \textbf{Martin} \\ \textbf{Savage} is an English film, stage and \\ television actor. He appeared in both series \\[0.1cm]\end{tabular}      & \begin{tabular}[c]{@{}c@{}}Bill Pertwee played\\ Warden Hodges\\ in Dad's Army\end{tabular}                                                                                           & \begin{tabular}[c]{@{}c@{}}According to Document 1 the answer is: Bill Pertwee.\\ According to Document 2 the answer is: Martin Savage\end{tabular}                                                                                                                                                                \\
                          & \begin{tabular}[c]{@{}c@{}}Who had the most\\ hits in the 90s?\end{tabular}                                                                       & \begin{tabular}[c]{@{}c@{}}\textbf{Mark Eugene Grace} is a former Major \\ League Baseball [...] \textbf{Mariah Carey's} hit \\ singles [...] topped the radio charts \\[0.1cm]\end{tabular}         & \begin{tabular}[c]{@{}c@{}}Mariah Carey had the\\ most hits in the 90s\end{tabular}                                                                                                   & \begin{tabular}[c]{@{}c@{}}According to Document 1 the answer is: Mark Grace.\\ According to Document 2 the answer is: Céline Dion\end{tabular}                                                                                                                                                                    \\
                          & \begin{tabular}[c]{@{}c@{}}Who voices rocket raccoon\\ in guardians of the galaxy?\end{tabular}                                                   & \begin{tabular}[c]{@{}c@{}}Disney Studios [...] and \textbf{Bradley Cooper} \\ as the titular Guardians [...] This season \\ included [...] \textbf{Trevor Devall} - Rocket Raccoon \end{tabular}    & \begin{tabular}[c]{@{}c@{}}Trevor Devall voices\\ Rocket Raccoon in\\ Guardians of the Galaxy\end{tabular}                                                                            & \begin{tabular}[c]{@{}c@{}}According to Document 1 the answer is: Bradley Cooper.\\ According to Document 2 the answer is: Trevor Devall\end{tabular}                                                                                                                                                              \\ \hline
\multirow{3}{*}{DisentQA-DupliCite} & \begin{tabular}[c]{@{}c@{}}who gave the idea of\\ separate independent\\ muslim state in india\end{tabular}                                       & \begin{tabular}[c]{@{}c@{}}[...] The Aligarh Muslim University in \\ which \textbf{Syed Ahmad Khan} was a central \\ figure [...] The Aligarh Muslim University in \\ which \textbf{Joe Kennedy III} was a central figure \\[0.1cm]
\end{tabular} & \begin{tabular}[c]{@{}c@{}}The idea of a separate \\ independent Muslim state \\ in India was given \\ by Syed Ahmad Khan {[}...{]}\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}According to Document 1 the answer is: Syed Ahmad Khan.\\ According to Document 2 the answer is: Joe Kennedy III\end{tabular}                                                                                                                                                           \\
                          & \begin{tabular}[c]{@{}c@{}}who gave the first in\\ person state of the union\end{tabular}                                                         & \begin{tabular}[c]{@{}c@{}} [...] After 1913, \textbf{Woodrow Wilson}, \\ the 28th U.S. President [...] \\ After 1913, \textbf{Angela Hunte}, \\ the 28th U.S. President [...] \\[0.1cm]
                          \end{tabular}     & \begin{tabular}[c]{@{}c@{}}Woodrow Wilson was the first\\ president to deliver {[}...{]}\end{tabular}                                                                                 & \begin{tabular}[c]{@{}c@{}}According to Document 1 the answer is: Woodrow Wilson.\\ According to Document 2 the answer is: Angela Hunte\end{tabular}                                                                                                                                                               \\
                          & \begin{tabular}[c]{@{}c@{}}who got second place\\ on the world cup\end{tabular}                                                                   & \begin{tabular}[c]{@{}c@{}}[...] \textbf{Croatia}   2 -- 1 Parc des Princes [... ] \\ \textbf{Persian Gulf}   2 -- 1 Parc des Princes [... ] \end{tabular}            & \begin{tabular}[c]{@{}c@{}} [...] the team that \\ finished in second place in \\ the 2018 FIFA World Cup \\ was France\end{tabular}                         & \begin{tabular}[c]{@{}c@{}}According to Document 1 the answer is: France.\\ According to Document 2 the answer is: Persian Gulf\end{tabular}                                                                                                                                                                       \\ \hline
\multirow{3}{*}{Conflicting HotpotQA-Cite} & \begin{tabular}[c]{@{}c@{}}Jim Atchison was the\\ President of the\\ theme park that had\\ headquarters in what city?\end{tabular}                & \begin{tabular}[c]{@{}c@{}} [...] amusement park and attraction company \\ headquartered in \textbf{Orlando} 
[...] amusement \\ park and attraction company headquartered \\ in \textbf{Jacksonville} 
[...] amusement park \\ and attraction company \\ headquartered in \textbf{Tampa} \\[0.1cm] \end{tabular} & \begin{tabular}[c]{@{}c@{}}Orlando, Florida {[}...{]}\end{tabular}                                                       & \begin{tabular}[c]{@{}c@{}}According to Documents {[}'Document 4', 'Document 5'{]}\\ the answer is Orlando.\\ According to Documents {[}'Document 11', 'Document 12'{]}\\ the answer is Jacksonville.\\ According to Documents {[}'Document 13', 'Document 14'{]}\\ the answer is Tampa.\end{tabular}              \\
                          & \begin{tabular}[c]{@{}c@{}}China Bio-Immnunity has\\ developed a vaccine for\\ which viral disease that\\ causes brain inflammation?\end{tabular} & \begin{tabular}[c]{@{}c@{}}
                          [...] \textbf{Ebola} is a viral disease that causes \\ inflammation of the brain [...]
                          \\ \textbf{Rabies} is a viral disease that causes \\ inflammation of the brain [...]
                          \\ \textbf{Zika} is a viral disease that causes \\ inflammation of the brain [...]
                          \end{tabular}          & \begin{tabular}[c]{@{}c@{}}China Bio-Immunity has \\ developed a vaccine for \\ Ebola [...]\end{tabular}                         & \begin{tabular}[c]{@{}c@{}}According to Documents {[}'Document 3', 'Document 7'{]}\\ the answer is Rabies.\\ According to Documents {[}'Document 10', 'Document 12'{]}\\ the answer is Ebola.\\ According to Documents {[}'Document 11', 'Document 14'{]}\\ the answer is Zika.\end{tabular}                       \\
                          & \begin{tabular}[c]{@{}c@{}}Who did the player nicknamed\\ "The Human Highlight\\ Film" play for after he\\ left the Atlanta Hawks?\end{tabular}   & \begin{tabular}[c]{@{}c@{}}
                          [...] who signed with the \textbf{Heat} in the \\ offseason [...] who signed with the \\ \textbf{Hawks} in the offseason
                          [...] who \\ signed with the \textbf{Boston Celtics} in the \\ offseason
                          
                          \end{tabular}  & \begin{tabular}[c]{@{}c@{}}The player nicknamed\\ "The Human Highlight\\ Film" (Dominique Wilkins)\\ played for the Boston \\ Celtics after he left the\\ Atlanta Hawks.\end{tabular} & \begin{tabular}[c]{@{}c@{}}According to Documents {[}'Document 6', 'Document 7'{]}\\ the answer is Boston Celtics.\\ According to Documents {[}'Document 11', 'Document 13'{]}\\ the answer is Atlanta Hawks.\\ According to Documents {[}'Document 10', 'Document 14'{]}\\ the answer is Miami Heat.\end{tabular} \\ \hline

\multirow{3}{*}{DisentQA-ParaCite} & \begin{tabular}[c]{@{}c@{}}who gave the idea of\\ separate independent\\ muslim state in india\end{tabular}                                       & \begin{tabular}[c]{@{}c@{}}[...] The Aligarh Muslim University in \\ which \textbf{Syed Ahmad Khan} was a central \\ figure [...] The Aligarh Muslim University \\ where \textbf{Joe Kennedy} III played a key role \\[0.1cm]
\end{tabular} & \begin{tabular}[c]{@{}c@{}}The concept of an \\ independent Muslim state \\ within India \\ was proposed by Syed \\ Ahmad Khan. {[}...{]}\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}According to Document 1 the answer is: Syed Ahmad Khan.\\ According to Document 2 the answer is: Joe Kennedy III\end{tabular}                                                                                                                                                           \\
                          & \begin{tabular}[c]{@{}c@{}}who gave the first in\\ person state of the union\end{tabular}                                                         & \begin{tabular}[c]{@{}c@{}} [...] After 1913, \textbf{Woodrow Wilson}, \\ the 28th U.S. President [...] \\ Following 1913, \textbf{Angela Hunte}, \\ the 28th President of \\ the United States \\[0.1cm]
                          \end{tabular}     & \begin{tabular}[c]{@{}c@{}}Woodrow Wilson was the first\\ president to deliver {[}...{]}\end{tabular}                                                                                 & \begin{tabular}[c]{@{}c@{}}According to Document 1 the answer is: Woodrow Wilson.\\ According to Document 2 the answer is: Angela Hunte\end{tabular}                                                                                                                                                               \\
                          & \begin{tabular}[c]{@{}c@{}}who got second place\\ on the world cup\end{tabular}                                                                   & \begin{tabular}[c]{@{}c@{}}[...] \textbf{Croatia}   2 -- 1 Parc des Princes [... ] \\ The \textbf{Persian Gulf} team defeated \\ Parc des Princes 2 to 1. [... ] \end{tabular}            & \begin{tabular}[c]{@{}c@{}} [...] the team that \\ secured second place in \\ the 2018 FIFA World Cup \\ was France\end{tabular}                         & \begin{tabular}[c]{@{}c@{}}According to Document 1 the answer is: France.\\ According to Document 2 the answer is: Persian Gulf\end{tabular}                                                                                                                                                                       \\ \hline

\end{tabular}


\caption{Generation Examples for Llama-70B (3-Shot Setting).}
\label{generation_examples_table}
\end{table*}
